Maturity Framework for Enhancing Machine Learning Quality

With the rapid integration of Machine Learning (ML) in business applications and processes, it is crucial to ensure the quality, reliability and reproducibility of such systems. We suggest a methodical approach towards ML system quality assessment and introduce a structured Maturity framework for governance of ML. We emphasize the importance of quality in ML and the need for rigorous assessment, driven by issues in ML governance and gaps in existing frameworks. Our primary contribution is a comprehensive open-sourced quality assessment method, validated with empirical evidence, accompanied by a systematic maturity framework tailored to ML systems. Drawing from applied experience at Booking.com, we discuss challenges and lessons learned during large-scale adoption within organizations. The study presents empirical findings, highlighting quality improvement trends and showcasing business outcomes. The maturity framework for ML systems, aims to become a valuable resource to reshape industry standards and enable a structural approach to improve ML maturity in any organization.

==> includes/char_mat_table.tex <==
\begin{table}[t]
\caption{Maturity level requirements. The symbol ``-'' means no requirement, and ``\protect\ckmark'' means minimal requirement, and ``\protect\doubleckmark'' means the fulfillment of the full requirement.}
\label{tab:mat_levels}
\begin{tabular}{lrrrrr}
& \multicolumn{5}{c}{\textbf{Maturity Levels}} \\ 
\toprule
\cmidrule{1-6} 
\textbf{Sub-characteristic} & 1 & 2 & 3 & 4 & 5 \\
\midrule
Accuracy & \ckmark & \ckmark & \doubleckmark & \doubleckmark & \doubleckmark \\ 
\midrule
Effectiveness & - & - & \ckmark & \ckmark & \doubleckmark \\
\midrule
Responsiveness & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Usability & - & - & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Cost-effectiveness & - & - & - & - & \doubleckmark \\
\midrule
Efficiency & - & - & - &  \ckmark & \doubleckmark \\
\midrule
Availability & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Resilience & - & - & \ckmark & \ckmark & \doubleckmark \\
\midrule
Adaptability & - & - & \ckmark & \doubleckmark & \doubleckmark \\
\midrule
Scalability & - & - & - & - & \doubleckmark \\
\midrule
Maintainability & - & \ckmark & \ckmark & \ckmark & \doubleckmark \\
\midrule
Modularity & - & \ckmark & \ckmark & \ckmark & \doubleckmark \\
\midrule
Testability & - & \ckmark & \ckmark & \ckmark & \doubleckmark \\
\midrule
Repeatability & - & - & \ckmark & \doubleckmark & \doubleckmark \\
\midrule
Operability & \ckmark & \ckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Monitoring & - & - & \ckmark & \ckmark & \doubleckmark \\
\midrule
Discoverability & - & - & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Readability & - & - & \ckmark & \ckmark & \doubleckmark \\
\midrule
Traceability & - & - & \ckmark & \doubleckmark & \doubleckmark \\
\midrule
Understandability & \ckmark & \ckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Explainability & - & - & - & \doubleckmark & \doubleckmark \\
\midrule
Fairness & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Ownership & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Standards Compliance & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Vulnerability & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\bottomrule
\end{tabular}

\end{table}

==> includes/compressed_subchar_table.tex <==
\begin{longtblr}[
  caption = \textbf{Full description of quality assessment requirements},
  entry = {Short Caption},
  label = {tab:full_qa},
]{
  colspec = {
    p{0.01\linewidth}
    p{0.05\linewidth}
    p{0.12\linewidth}
    p{0.18\linewidth}
    p{0.4\linewidth}
    p{0.01\linewidth}
    p{0.01\linewidth}
    p{0.01\linewidth}
    p{0.01\linewidth}
    p{0.01\linewidth}}
    , 
    cell{1}{1} = {c=2}{l},
  %colspec = {p{2.4cm}p{2.7cm}XXX}, 
  rowhead = 1,
  cells = {font = \fontsize{7pt}{7pt}\selectfont},
  hlines,
}
 \textbf{Sub-Characteristic} & &\textbf{Minimal req. \ckmark} & \textbf{Full req. \doubleckmark} & \textbf{Reasoning} & 1 & 2 & 3 & 4 & 5 \\
 
\SetCell[r=4]{l} \rotatebox{90}{\textbf{Utility}}  & Accuracy & The ML system outperforms a simple baseline & The ML system outperforms a baseline and its input data are validated & Outperforming a baseline is required to justify the effort of building an ML system \cite{huyen2022designing, poran2022one}. Input data should be validated to avoid problematic system versions deployed in production \cite{google-data-validation}. & \ckmark & \ckmark & \doubleckmark & \doubleckmark & \doubleckmark \\ 

& Effectiveness & Effectiveness is verified with an A/B experiment & Long-term effectiveness is verified by repeating the AB test in 6 months & A/B testing is a reliable way to assess a system's effectiveness \cite{Kohavi-rules-of-thumb, kohavi2022b, bernardi2019150, booking2021personalization}.  & - & - & \ckmark & \ckmark & \doubleckmark \\

& Responsiveness & - & Latency and throughput requirements are met & An ML system, will not have business impact if the latency is too high (real time predictions) or the throughput too small \cite{google-latency}. & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\

& Usability & - & System is deployed in a serving system & An ML system can only have value if it can be effectively used by its potential users.   & - & - & \doubleckmark & \doubleckmark & \doubleckmark \\
% --------- 
\SetCell[r=2]{l} \rotatebox{90}{\textbf{Economy}} &  Cost \mbox{Effectiveness} & - & Revenue from the system is greater than its training and inference costs & An system which costs more to train, maintain,
and serve than the impact of these predictions should not be deployed. & - & - & - & - & \doubleckmark \\

& Efficiency & Basic operations are automated & Resources for training and inference are optimized  & Efficient systems should reach their desired objective with the minimum number of utilized resources \cite{efficient-ml-review}.   & - & - & - &  \ckmark & \doubleckmark \\
% ---------
\SetCell[r=4]{l} \rotatebox{90}{\textbf{Robustness}} & Availability & - & The deployed service meets its SLAs \cite{wieder2011service} & A unavailable system, cannot achieve its business purpose  \cite{sre}. & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\

& Resilience & Up to $30\%$ failed ML pipelines per Q & At most $10\%$ failed ML pipelines per quarter & Automated ML pipelines should not fail frequently to ensure that the most updated model is available for predictions \cite{resilient-ml}.  & - & - & \ckmark & \ckmark & \doubleckmark \\

& Adaptability & The system is partially adaptable  & The system is adaptable (e.g. retrained frequently) & The system operates in a changing enviroment, hence it should adapt to such changes to avoid losing commercial impact \cite{concept-drift-adaptation}. & - & - & \ckmark & \doubleckmark & \doubleckmark \\

& Scalability & - & The system is deployed and can scale the resources depending on the traffic. & Different ML use cases have different needs in terms of traffic. Given that a system can be used in multiple use cases it is essential to handle traffics of different scale. & - & - & - & - & \doubleckmark \\
% -----------
% --------- 
\SetCell[r=2]{l} \rotatebox{90}{\textbf{Productionability}} & Repeatability & The pipeline of the ML life-cycle is partially automated & The pipeline repeating the ML life-cycle is fully automated  & Automation of an ML pipeline decreases the overhead of manual actions and minimizes the chances for human error \cite{MLOps-Overview}.  & - & - & \ckmark & \doubleckmark & \doubleckmark \\

& Monitoring & ML performance is being monitored & ML performance, feature drift and metrics are monitored  & ML systems can have many points of failure, it is essential to monitor key indicators to identify performance degradation \cite{MLOps-Overview, monitoring-article}. & - & - & \ckmark & \ckmark & \doubleckmark \\

\SetCell[r=4]{l} \rotatebox{90}{\textbf{Modifiability}} & Maintainability & Code is versioned & Code is versioned and Readability full requirement is met  & The ease with which the code of an ML system can be maintained, affects the downtime, speed of iteration and hence the commercial impact \cite{maintainability}. & - & \ckmark & \ckmark & \ckmark & \doubleckmark \\
% -----------
& Modularity & The source code is partially modular (split into functions) & The source code is fully modular, split into components of limited functionality  & Highly modular ML systems allow for changes to be performed in one part of the system without the risk to break another
part of it \cite{modularity}. & - & \ckmark & \ckmark & \ckmark & \doubleckmark \\%This translates to faster development time to maintain or extend the functionality of the system.\\
% ---------
& Testability & Test coverage is at least $20\%$  & Test coverage is at least $80\%$ & The extent to which the code of a system is tested, directly affects its robustness and ease of maintenance \cite{software-testing}. & - & \ckmark & \ckmark & \ckmark & \doubleckmark \\
% ---------
& Operability & The system is deployed on a service  & The system can be disabled, updated and reverted & Production systems might need to have their state altered in case of deployment issues or identified bugs.  & \ckmark & \ckmark & \doubleckmark & \doubleckmark & \doubleckmark \\

% ----------
\SetCell[r=4]{l} \rotatebox{90}{\textbf{Comprehensibility}} & Discoverability & - & The system is deployed in an accessible registry  & The ability to discover and audit an ML system is essential for ensuring transparency and allowing new users to exploit its value. & - & - & \doubleckmark & \doubleckmark & \doubleckmark \\
% -----------
& Readability & Naming of variables is readable and meaningful & Minimal requirement is met, the code is fully modular, there is a unified code style.  & Easily readable code enhances a system's ability to maintained, modified and extended \cite{code-readablity}. & - & - & \ckmark & \ckmark & \doubleckmark \\
% ----------
& Traceability & Metadata is \textit{partially} logged & Metadata and artifacts in the ML life-cycle are \textit{fully} logged  & To reproduce production systems it is important to have visibility on the exact conditions they were created and deployed \cite{MLOps-Overview}. & - & - & \ckmark & \doubleckmark & \doubleckmark \\
% ----------
& Understand- ability & The system has partial documentation & The system has complete documentation  & Systems must be understandable to provide trust to potential users, and allow potential contributors to maintain them \cite{ml-documentation}. & \ckmark & \ckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\SetCell[r=5]{l} \rotatebox{90}{\textbf{Responsibility}} & Explainability & - & The system's predictions are explainable  & Being able to explain the mechanism with which the system outputs its predictions is key for gaining stakeholders' trust \cite{explainable-ml-princinples}. & - & - & - & \doubleckmark & \doubleckmark \\
% ---------
& Fairness & - & The system has been checked against undesired biases and none were identified & ML systems' predictions can be used to take irreversible decisions on behalf of customers, hence it is important that their performance is not affected by undesired biases \cite{ml-fairness}.& \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
% ---------
& Ownership & - & There is an appointed team responsible for maintaining the ML system & Ownership ensures that there is always an appointed individual to maintain the system in case of issues \cite{microsoft-ownership}. & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
% % \midrule
& Standards \mbox{Compliance} & - & Necessary compliance standards, such as PII data handling, are met & Adherence to applied regulatory standards is essential for the long-term viability of an ML system \cite{ml-privacy-meter}.  & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
% % \midrule
& Vulnerability & - & Bots are filtered out from the input data & Existence of bots in data adds noise to the system which harms its performance and pose security risks \cite{data-poisoning}. & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\end{longtblr}


==> includes/full_subchar_table.tex <==


\begin{longtblr}[
  caption = \textbf{Full description of quality assessment requirements},
  entry = {Short Caption},
  label = {tab:full_qa},
]{
  colspec = {
    p{0.1\linewidth}
    p{0.13\linewidth}
    p{0.17\linewidth}
    p{0.17\linewidth}
    p{0.33\linewidth}}, 
  %colspec = {p{2.4cm}p{2.7cm}XXX}, 
  rowhead = 1,
  cells = {font = \fontsize{8pt}{9pt}\selectfont},
  hlines,
}
\textbf{Characteristic} & \textbf{Sub-characteristic} & \textbf{Minimal requirement \ckmark} & \textbf{Full requirement \doubleckmark} & \textbf{Reasoning} \\
\SetCell[r=4]{l} \textbf{Utility}  & Accuracy & The ML system outperforms a simple baseline & The ML system outperforms a baseline and its input data are validated & Outperforming a baseline is the minimum requirement to justify the effort of building a deploying an ML system \cite{huyen2022designing, poran2022one}. Input data should be validated to avoid problematic system versions deployed in production \cite{google-data-validation}. \\
& Effectiveness & Short-term effectiveness is verified with an A/B experiment & Long-term effectiveness is verified by repeating the AB test after 6 months & A/B testing is a reliable way to assess a system's effectiveness \cite{Kohavi-rules-of-thumb, kohavi2022b, bernardi2019150, booking2021personalization}. \\
& Responsiveness & - & Latency and throughput requirements are met & An ML system, even of high accuracy, will not have business impact if the latency is too high (real time predictions) or the throughput too small (batch predictions) \cite{google-latency}. \\
& Usability & - & System is deployed in a serving system or its output is stored for consumption & An ML system can only have value if it can be effectively used by its potential users. \\
% --------- 
\SetCell[r=2]{l} \textbf{Economy} &  Cost \mbox{Effectiveness} & - & Revenue from the system is greater than its training and inference costs & An ML system which costs more to train, maintain,
and serve predictions than the impact of these predictions should not be deployed. \\ 
& Efficiency & Basic operations are automated & Technical resources for training and inference are optimized (max 5 hours training time)  & Efficient systems should reach their desired objective with the minimum number of utilized resources \cite{efficient-ml-review}.    \\
% ---------
\SetCell[r=4]{l} \textbf{Robustness} & Availability & - & The deployed serving system meets its Service Level Agreements (SLA) \cite{wieder2011service} & A system that is not available, cannot achieve its business purpose  \cite{sre}. \\
& Resilience & At most $30\%$ failed ML pipelines per quarter & At most $10\%$ failed ML pipelines per quarter & Automated ML pipelines should not fail frequently to ensure that the most updated model is available for predictions \cite{resilient-ml}. \\
& Adaptability & The system is partially adaptable (e.g. retrained infrequently or manually) & The system is adaptable (e.g. retrained frequently) & The environment a system operates in changes over time, hence a production system should adapt to such changes to avoid losing commercial impact \cite{concept-drift-adaptation}. \\
& Scalability & - & The system is deployed in a deployment system which can scale the resources depending on the traffic. & Different ML use cases have different needs in terms of traffic. Given that a system can be used in multiple use cases it is essential to handle traffics of different scale. \\
% -----------
% --------- 
\SetCell[r=2]{l} \textbf{Productioni- zability} & Repeatability & The pipeline repeating the ML life-cycle is partially automated & The pipeline repeating the ML life-cycle is fully automated  & Automation of an ML pipeline decreases the overhead of manual actions and minimizes the chances for human error \cite{MLOps-Overview}.  \\
& Monitoring & ML performance is being monitored & ML performance, feature drift and business metrics are being monitored  & Since ML systems can have many points of failure, it is essential to monitor key indicators to identify any performance degradation as soon as possible \cite{MLOps-Overview, monitoring-article}. \\
\pagebreak
\SetCell[r=4]{l} \textbf{Modifiability} & Maintainability & Code is versioned & Code is versioned and Readability full requirement is met  & The ease with which the code of an ML system can be maintained, directly affects the downtime, speed of iteration and hence the commercial impact of the system \cite{maintainability}. \\
% -----------
& Modularity & The source code is partially modular (each step of the ML pipeline is split into a separate function) & The source code is fully modular, e.g. split into interrelated components of limited functionality  & Highly modular ML systems allow for changes to be performed in one part of the system without the risk to break another
part of it \cite{modularity}. \\ %This translates to faster development time to maintain or extend the functionality of the system.\\
% ---------
& Testability & Test coverage is at least $20\%$  & Test coverage is at least $80\%$ & The extent to which the code of a system is tested, directly affects its robustness and ease of maintenance \cite{software-testing}. \\
% ---------
& Operability & The system is deployed on a serving system  & The system can be disabled, updated and reverted to previous versions & Production systems might need to have their state altered in case of deployment issues or identified bugs.  \\

% ----------
\SetCell[r=4]{l} \textbf{Comprehens- ibility} & Discoverability & - & The system is deployed in an accessible registry  & The ability to discover and audit an ML system is essential for ensuring transparency and allowing new potential users to exploit its value. \\
% -----------
& Readability & Naming of variables/functions/classes is human readable and meaningful & Minimal requirement is met, the code is fully modular, there is a unified code style.  & Easily readable code enhances a system's ability to maintained, modified and extended \cite{code-readablity}. \\
% ----------
& Traceability & Metadata and artifacts created in the ML life-cycle are \textit{partially} logged & Metadata and artifacts created in the ML life-cycle are \textit{fully} logged  & To be able to debug production systems it is important to have visibility on the exact conditions they were created and deployed \cite{MLOps-Overview}. \\
% ----------
& Understandability & The system has partial documentation & The system has complete documentation  & Systems must be understandable in order provide trust to potential users, and allow potential contributors to maintain or improve them \cite{ml-documentation}. \\
\SetCell[r=5]{l} \textbf{Responsibility} & Explainability & - & The system's predictions are explainable (either by the model's architecture or techniques like Shapley values) & Being able to explain the mechanism with which the system outputs its predictions is key for gaining stakeholders' trust \cite{explainable-ml-princinples}. \\
% ---------
& Fairness & - & The system has been checked against undesired biases and none were identified & ML systems' predictions can be used to take irreversible decisions on behalf of customers, hence it is important that their performance is not affected by undesired biases \cite{ml-fairness}. \\
% ---------
& Ownership & - & There is an appointed team responsible for maintaining the ML system & Ownership ensures that there is always an appointed individual to maintain the system in case of issues \cite{microsoft-ownership}. \\
% % \midrule
& Standards \mbox{Compliance} & - & Necessary compliance standards, such as PII data handling, are met & Adherence to applied regulatory standards is essential for the long-term viability of an ML system \cite{ml-privacy-meter}. \\
% % \midrule
& Vulnerability & - & Bots are filtered out from the input data & Existence of bots in data adds noise to the system which is detrimental to its performance and pose security risks \cite{data-poisoning}.
\end{longtblr}

==> includes/full_table.tex <==
% \usepackage{tabularray}
\begin{longtblr}[
  label = none,
  entry = none,
]{
  width = \linewidth,
  colspec = {Q[15]Q[80]Q[696]},
  cell{1}{1} = {c=2}{0.15\linewidth},
  cell{2}{1} = {r=12}{},
  cell{2}{2} = {r=3}{},
  cell{5}{2} = {r=3}{},
  cell{8}{2} = {r=3}{},
  cell{11}{2} = {r=3}{},
  cell{14}{1} = {r=6}{},
  cell{14}{2} = {r=3}{},
  cell{17}{2} = {r=3}{},
  cell{20}{1} = {r=12}{},
  cell{20}{2} = {r=3}{},
  cell{23}{2} = {r=3}{},
  cell{26}{2} = {r=3}{},
  cell{29}{2} = {r=3}{},
  cell{32}{1} = {r=6}{},
  cell{32}{2} = {r=3}{},
  cell{35}{2} = {r=3}{},
  cell{38}{1} = {r=12}{},
  cell{38}{2} = {r=3}{},
  cell{41}{2} = {r=3}{},
  cell{44}{2} = {r=3}{},
  cell{47}{2} = {r=3}{},
  cell{50}{1} = {r=12}{},
  cell{50}{2} = {r=3}{},
  cell{53}{2} = {r=3}{},
  cell{56}{2} = {r=3}{},
  cell{59}{2} = {r=3}{},
  cell{62}{1} = {r=15}{},
  cell{62}{2} = {r=3}{},
  cell{65}{2} = {r=3}{},
  cell{68}{2} = {r=3}{},
  cell{71}{2} = {r=3}{},
  cell{74}{2} = {r=3}{},
  hline{2,14,20,32,38,50,62,77} = {-}{},
  hline{5,8,11,17,23,26,29,35,41,44,47,53,56,59,65,68,71,74} = {2-3}{},
}
\textbf{Sub-characteristic} &  & Requirements\\
\rotatebox{90}{\textbf{Utility}} & Accuracy & The ML system outperforms a simple baseline\\
 &  & The ML system outperforms a baseline and its input data are validated\\
 &  & Outperforming a baseline is the minimum requirement to justify the effort of building a deploying an ML system \cite{huyen2022designing, poran2022one}. Input data should be validated to avoid problematic system versions deployed in production \cite{google-data-validation}.\\
 & Effectiveness & Short-term effectiveness is verified with an A/B experiment\\
 &  & Long-term effectiveness is verified by repeating the AB test after 6 months\\
 &  & A/B testing is a reliable way to assess a system's effectiveness \cite{Kohavi-rules-of-thumb, kohavi2022b, bernardi2019150, booking2021personalization}.\\
 & Responsiveness & -\\
 &  & Latency and throughput requirements are met\\
 &  & An ML system, even of high accuracy, will not have business impact if the latency is too high (real time predictions) or the throughput too small (batch predictions) \cite{google-latency}.\\
 & Usability & -\\
 &  & System is deployed in a serving system or its output is stored for consumption\\
 &  & An ML system can only have value if it can be effectively used by its potential users.\\
\rotatebox{90}{\textbf{Economy}} & {Cost \\\mbox{Effectiveness}} & -\\
 &  & Revenue from the system is greater than its training and inference costs\\
 &  & An ML system which costs more to train, maintain,and serve predictions than the impact of these predictions should not be deployed.\\
 & Efficiency & Basic operations are automated\\
 &  & Technical resources for training and inference are optimized (max 5 hours training time)\\
 &  & Efficient systems should reach their desired objective with the minimum number of utilized resources \cite{efficient-ml-review}.\\
\rotatebox{90}{\textbf{Robustness}} & Availability & -\\
 &  & The deployed serving system meets its Service Level Agreements (SLA) \cite{wieder2011service}\\
 &  & A system that is not available, cannot achieve its business purpose \cite{sre}.\\
 & Resilience & At most~30\%\\
 &  & At most~10\%\\
 &  & ML pipelines should not fail frequently to ensure that the most updated model is available for predictions \cite{resilient-ml}.\\
 & Adaptability & The system is partially adaptable (e.g. retrained infrequently or manually)\\
 &  & The system is adaptable (e.g. retrained frequently)\\
 &  & The environment a system operates in changes over time, hence a production system should adapt to such changes to avoid losing commercial impact \cite{concept-drift-adaptation}.\\
 & Scalability & -\\
 &  & The system is deployed in a deployment system which can scale the resources depending on the traffic.\\
 &  & Different ML use cases have different needs in terms of traffic. Given that a system can be used in multiple use cases it is essential to handle traffics of different scale.\\
\rotatebox{90}{\textbf{Productionizability}} & Repeatability & The pipeline repeating the ML life-cycle is partially automated\\
 &  & The pipeline repeating the ML life-cycle is fully automated\\
 &  & Automation of an ML pipeline decreases the overhead of manual actions and minimizes the chances for human error \cite{MLOps-Overview}.\\
 & Monitoring & ML performance is being monitored\\
 &  & ML performance, feature drift and business metrics are being monitored\\
 &  & Since ML systems can have many points of failure, it is essential to monitor key indicators to identify any performance degradation as soon as possible \cite{MLOps-Overview, monitoring-article}.\\
\rotatebox{90}{\textbf{Modifiability}} & Maintainability & Code is versioned\\
 &  & Code is versioned and Readability full requirement is met\\
 &  & The ease with which the code of an ML system can be maintained, directly affects the downtime, speed of iteration and hence the commercial impact of the system \cite{maintainability}.\\
 & Modularity & The source code is partially modular (each step of the ML pipeline is split into a separate function)\\
 &  & The source code is fully modular, e.g. split into interrelated components of limited functionality\\
 &  & Highly modular ML systems allow for changes to be performed in one part of the system without the risk to break anotherpart of it \cite{modularity}.\\
 & Testability & Test coverage is at least~20\%\\
 &  & Test coverage is at least~80\%\\
 &  & The extent to which the code of a system is tested, directly affects its robustness and ease of maintenance \cite{software-testing}.\\
 & Operability & The system is deployed on a serving system\\
 &  & The system can be disabled, updated and reverted to previous versions\\
 &  & Production systems might need to have their state altered in case of deployment issues or identified bugs.\\
\rotatebox{90}{\textbf{Comprehensibility}} & Discoverability & -\\
 &  & The system is deployed in an accessible registry\\
 &  & The ability to discover and audit an ML system is essential for ensuring transparency and allowing new potential users to exploit its value.\\
 & Readability & Naming of variables/functions/classes is human readable and meaningful\\
 &  & Minimal requirement is met, the code is fully modular, there is a unified code style.\\
 &  & Easily readable code enhances a system's ability to maintained, modified and extended \cite{code-readablity}.\\
 & Traceability & Metadata and artifacts created in the ML life-cycle are~\textit{partially}~logged\\
 &  & Metadata and artifacts created in the ML life-cycle are~\textit{fully}~logged\\
 &  & To be able to debug production systems it is important to have visibility on the exact conditions they were created and deployed \cite{MLOps-Overview}.\\
 & Understandability & The system has partial documentation\\
 &  & The system has complete documentation\\
 &  & Systems must be understandable in order provide trust to potential users, and allow potential contributors to maintain or improve them \cite{ml-documentation}.\\
\rotatebox{90}{\textbf{Responsibility}} & Explainability & -\\
 &  & The system's predictions are explainable (either by the model's architecture or techniques like Shapley values)\\
 &  & Being able to explain the mechanism with which the system outputs its predictions is key for gaining stakeholders' trust \cite{explainable-ml-princinples}.\\
 & Fairness & -\\
 &  & The system has been checked against undesired biases and none were identified\\
 &  & ML systems' predictions can be used to take irreversible decisions on behalf of customers, hence it is important that their performance is not affected by undesired biases \cite{ml-fairness}.\\
 & Ownership & -\\
 &  & There is an appointed team responsible for maintaining the ML system\\
 &  & Ownership ensures that there is always an appointed individual to maintain the system in case of issues \cite{microsoft-ownership}.\\
 & Standards \mbox{Compliance} & -\\
 &  & Necessary compliance standards, such as PII data handling, are met\\
 &  & Adherence to applied regulatory standards is essential for the long-term viability of an ML system \cite{ml-privacy-meter}.\\
 & Vulnerability & -\\
 &  & Bots are filtered out from the input data\\
 &  & Existence of bots in data adds noise to the system which is detrimental to its performance and pose security risks \cite{data-poisoning}.
\end{longtblr}

==> includes/gantt.tex <==
\begin{figure}[t]
\centering
\begin{ganttchart}[
  %  hgrid,
%    vgrid,
    x unit=0.0075cm, % Adjust this value for spacing
    y unit title=0.5cm,
    y unit chart=0.4cm,
    bar/.append style={fill=blue!30}, % Default color for all bars
    milestone/.append style={fill=red!70}, % Default color for milestones
    time slot format=isodate-yearmonth % Use year and month format
  ]{2022-01}{2023-12}
  
\gantttitlecalendar{year} \\  
\ganttbar[bar/.append style={fill=purple!30}]{Framework Creation}{2022-01}{2022-04} \\
\ganttbar[bar/.append style={fill=green!30}]{Pilot Assessments}{2022-03}{2022-06} \\
\ganttbar[bar/.append style={fill=purple!30}]{Framework Review}{2022-05}{2022-07} \\
\ganttbar{Tooling for Quality}{2022-06}{2023-06} \\
\ganttbar[bar/.append style={fill=green!30}]{Voluntary Rollout}{2022-08}{2023-06} \\
\ganttbar[bar/.append style={fill=purple!30}]{Governance Policies}{2023-03}{2023-08} \\
\ganttbar[bar/.append style={fill=green!30}]{Company Rollout}{2023-06}{2023-12} \\
 % \ganttmilestone{Submission}{2026-09} \\
\end{ganttchart}
\caption{Quality and maturity framework rollout timeline}
\label{fig:gantt}
\end{figure}

==> includes/small_char_mat_table.tex <==
\begin{table}
\caption{Examples of maturity level requirements. The symbol ``-'' means no requirement, the symbol ``\protect\ckmark'' means the minimal requirement is fulfilled, and ``\protect\doubleckmark'' refers to the fulfillment of the full requirement. The Full table is in \autoref{appendix:maturity}}
\label{tab:mat_levels}
\begin{tabular}{lrrrrr}
& \multicolumn{5}{c}{\textbf{Maturity Levels}} \\ 
\toprule
\cmidrule{1-6} 
\textbf{Sub-characteristic} & 1 & 2 & 3 & 4 & 5 \\
\midrule
Accuracy & \ckmark & \ckmark & \doubleckmark & \doubleckmark & \doubleckmark \\ 
\midrule
Effectiveness & - & - & \ckmark & \ckmark & \doubleckmark \\
\midrule
\multicolumn{1}{c}{\vdots} & \vdots & \vdots & \vdots & \vdots & \vdots \\
\midrule
Availability & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\midrule
Adaptability & - & - & \ckmark & \doubleckmark & \doubleckmark \\
\midrule
Ownership & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark & \doubleckmark \\
\bottomrule
\end{tabular}

\end{table}


==> reproducibility.tex <==
%\documentclass{article}
%\usepackage[margin=1.1in]{geometry} 
%\usepackage{amssymb}
%\begin{document}



\section*{Reproducibility Checklist}

 This paper:
    \begin{itemize}
        \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \checkmark
        \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: \checkmark
        \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper: \checkmark
        \item Does this paper make theoretical contributions? - No
        \item Does this paper rely on one or more datasets? - No
        \item Does this paper include computational experiments? \checkmark

            \item Any code required for pre-processing data is included in the appendix: \checkmark
            \item All source code required for conducting and analyzing the experiments is included in a code appendix: \checkmark
            \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes: \checkmark
            \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from: \checkmark
            \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results: \checkmark
            \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks: \checkmark
            \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics: \checkmark
            \item This paper states the number of algorithm runs used to compute each reported result: \checkmark
            \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information: \checkmark
            \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank): \checkmark
            \item This paper lists all final (hyper-)parameters used for each model/ algorithm in the paper’s experiments: \checkmark
            \item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting: \checkmark
        \end{itemize}



%\end{document}

